The *-variation of the Banach-Mazur game and forcing axioms

We introduce a property of posets which strengthens (\omega_1+1)-strategic closedness. This property is defined using a variation of the Banach-Mazur game on posets, where the first player chooses a countable set of conditions instead of a single condition at each turn. We prove PFA is preserved under any forcing over a poset with this property. As an application we reproduce a proof of Magidor's theorem about the consistency of PFA with some weak variations of the square principles. We also argue how different this property is from (\omega_1+1)-operational closedness, which we introduced in our previous work, by observing which portions of MA^+(\omega_1-closed) are preserved or destroyed under forcing over posets with either property.

==> setdefs.tex <==
%%写像
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\onetoone}{\rightarrowtail}
\newcommand{\restrict}{\upharpoonright}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\ran}{\mathrm{ran}}
%%論理
\newcommand{\equivalent}{{\ \Leftrightarrow\ }}
\newcommand{\imply}{{\ \Rightarrow\ }}
\newcommand{\revimpl}{{\ \Leftarrow\ }}
%%集合論
\newcommand{\force}{\Vdash}
\newcommand{\cf}{\mathrm{cf}}
\newcommand{\power}{\mathcal{P}}
\newcommand{\ro}{\mathrm{r.o.}}
\newcommand{\boolel}{[}%要変更
\newcommand{\booler}{]}%要変更
\newcommand{\Ord}{\mathrm{Ord}}
%%列
\newcommand{\concat}[2]{{{#1}^\smallfrown#2}}
\newcommand{\seq}[1]{{\langle#1\rangle}}
\newcommand{\lh}{\mathrm{lh}}
%%頻出文字
\renewcommand{\P}{{\mathbb P}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\V}{{\mathbf V}}


